Design and Implement an Enhanced Simulator for Autonomous Delivery Robot

As autonomous driving technology is getting more and more mature today, autonomous delivery companies like Starship, Marble, and Nuro has been making progress in the tests of their autonomous delivery robots. While simulations and simulators are very important for the final product landing of the autonomous delivery robots since the autonomous delivery robots need to navigate on the sidewalk, campus, and other urban scenarios, where the simulations can avoid real damage to pedestrians and properties in the real world caused by any algorithm failures and programming errors and thus accelerate the whole developing procedure and cut down the cost. In this case, this study proposes an open-source simulator based on our autonomous delivery robot ZebraT to accelerate the research on autonomous delivery. The simulator developing procedure is illustrated step by step. What is more, the applications on the simulator that we are working on are also introduced, which includes autonomous navigation in the simulated urban environment, cooperation between an autonomous vehicle and an autonomous delivery robot, and reinforcement learning practice on the task training in the simulator. We have published the proposed simulator in Github.

==> content/03_Architecture.tex <==
\section{Architecture}
\label{sec:Architecture}
If 
\weisong{give more details about xxxxx}

\begin{equation}
\begin{array}{c}
  S = \binom{N}{n},A_{k} = \binom{M}{k}\cdot \binom{N-M}{n-k} \\ \\
  P\left ( A_{k}\right ) = \frac{\binom{M}{k}\cdot \binom{N-M}{n-k}}{\binom{N}{n}} 
\end{array}
\end{equation}

Use the following web tool to get the formula in latex format:
\href{https://www.latexlive.com/}{https://www.latexlive.com/} 

==> content/04_CaseStudy.tex <==
\section{Case Study}
\label{sec:case}
In this section, we give several case studies where edge
computing could shine to further illustrate our vision of edge
computing.

\subsection{Cloud Offloading}
\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figures/Equinox.pdf}
\caption{Insert a figure.}
\label{system-design}
\end{figure}

In the traditional content delivery network, only the data is
cached at the edge servers. This is based on the fact that the
content provider provides the data on the Internet, which is
true for the past decades. In the IoT, the data is produced and
consumed at the edge. Thus, in the edge computing paradigm,
not only data but also operations applied on the data should
be cached at the edge.

\subsection{Video Analytics}
The widespread of mobilephones and network cameras
make video analytics an emerging technology. Cloud computing is no longer suitable for applications that requires video
analytics due to the long data transmission latency and privacy
concerns. Here we give an example of finding a lost child
in the city.

==> content/05_Comparison.tex <==
\section{Comparison}
\label{sec:evaluation}
This section provides a comparison of different simulators described under Section 4, starting with MATLAB, CarSim and PreScan. Then we compare Gazebo and CARLA, followed by comparison of CARLA and LGSVL. Finally, we conclude with our analysis and key observations.

MATLAB/Simulink is designed for the simple scenarios. It is good at computation and has efficient plot functions. The capability of co-simulation with other software like CarSim makes it  easier to build various vehicle models. It is common to see users using the vehicle models from CarSim and build their upper control algorithms in MATLAB/Simulink to do a co-simulation project. However, MATLAB/Simulink has limited ability to realistically visualize the traffic scenarios, obstacles and pedestrian models. PreScan has strong capability to simulate the environment of the real world such as the weather conditions that MATLAB/Simulink and CarSim cannot do, it also has interfaces with MATLAB/Simulink that makes modelling more efficient.

Further, Gazebo is known for its high flexibility and its seamless integration with ROS. While the high flexibility is advantageous because it gives full control over simulation, it comes at a cost of time and effort. As opposed to CARLA and LGSVL simulators, the creation of a simulation world in Gazebo is a manual process where the user must create 3D models and carefully define their physics and their position in the simulation world within the XML file. Gazebo does include various sensor models and it allows users to create new sensor models via the plugins. Next, we compare CARLA and LGSVL simulators. 

Both CARLA and LGSVL provide high quality simulation environments that require GPU computing unit in order to run with reasonable performance and frame rate.  The user can invoke different facilities in CARLA and LGSVL via using a flexible API. Although, the facilities are different between two simulators. For instance, CARLA provides build-in recorder while LGSVL does not provide. Therefore, in order to record videos in LGSVL, the user can leverage video recording feature in Nvidia drivers. CARLA and LGSVL provide a variety of sensors, some of these sensors are common between them such as  Depth camera, Lidar, and IMU. In addition, each simulator provides different sensors with description provided in their official website. Both simulators, CARLA and LGSVL, enhance users to create the custom sensors. The new map generation has different process in CARLA and LGSVL. The backbone of CARLA simulator is Unreal Engine that generates new maps by automatically adding stop signs based on the OpenDRIVE technology. On the other hand, the backbone of LGSVL simulator is Unity game engine and user can generate new map by manually importing different components into the Unity game engine. Additionally, the software architecture in CARLA and LGSVL is quite different. LGSVL mostly connects to AD stacks (Autoware, Apollo, and etc. ) based on different bridges and most of the simulators' facilities publishes or subscribes the data on specified topics in order to enables AD stacks to consume data. On the other hand, most of facilities in CARLA are built in, although it enables users to connects to ROS1,ROS2, and Autoware via using the bridges. 


While all of the six simulators described in the paper offer their own advantages and disadvantages, we make the following key observations. 
\begin{itemize}
  \item \textbf{\emph{Observation 1:}} LGSVL and CARLA are most suited for end to end testing of unique functionalities that self-driving cars offer such as perception, mapping, localization, and vehicle control because of many built-in automated features they support.
  \item \textbf{\emph{Observation 2:}} Gazebo is a popular robotic simulator but the time and effort needed to create dynamic scenes does not make it the first choice for testing end to end systems for self-driving cars
  \item \textbf{\emph{Observation 3:}} MATLAB/Simulink is one of the best choices for testing upper level algorithms because of the clearly presented logic blocks in Simulink. Additionally, it has a fast plot function that makes it easier to do the results analysis.
  \item \textbf{\emph{Observation 4:}} CarSim specializes in vehicle dynamic simulations because of its complete vehicle library and variety of vehicle parameters available to tune. However, it has limited ability to build customized upper-level algorithms in an efficient way.
  \item \textbf{\emph{Observation 5:}} PreScan has a strong capability of building realistic environments and simulating different weather conditions.
\end{itemize}


In Table~\ref{tab:comparison}, we provide a comparison summary where all six simulators described in this paper are further compared.

\begin{table*}[h!]
\caption{Comparison of various simulators.}
\label{tab:comparison}
\centering
\begin{tabular}{|p{0.15\linewidth}||p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|}
\hline
\textbf{Requirements} & \textbf{MATLAB (Simulink)} & \textbf{CarSim} & \textbf{PreScan} & \textbf{CARLA} & \textbf{Gazebo} & \textbf{LGSVL}\\
\hline
\hline
\textbf{Perception}: Sensor models supported & Y & Y  & Y & Y(1) & Y(2) & Y(3) \\
\hline
\textbf{Perception}: support for different weather conditions & N & N  & Y  & Y & N & Y \\
\hline
\textbf{Camera Calibration} & Y & N  & Y & Y & N  & N \\
\hline
\textbf{Path Planning} & Y & Y  & Y  & Y & Y & Y \\
\hline
\textbf{Vehicle Control}: Support for proper vehicle dynamics & Y & Y  & Y  & Y & Y & Y(3) \\
\hline

\textbf{3D Virtual Environment} & U & Y  & Y  & Y, Outdoor (Urban) & Y, Indoor and Outdoor & Y, Outdoor (Urban)\\
\hline
\textbf{Traffic Infrastructure} & Y, allows to build lights model & Y  & Y & Y, Traffic lights, Intersections, Stop signs, lanes  & Y, allows to manually build all kinds of models & Y\\
\hline
\textbf{Traffic Scenario simulation}: Support of different types of Dynamic objects & Y & Y & Y & Y & N(2) & Y \\
\hline
\textbf{2D/3D Ground Truth} & Y & N & N & Y & U & Y\\
\hline
\textbf{Interfaces to other software} & Y,  with Carsim, Prescan,ROS & Y, with Matlab(Simulink) & Y, with MATLAB(Simulink) & Y, with ROS, Autoware & Y, with ROS & Y, with Autoware, Apollo, ROS\\
\hline
\textbf{Scalability} via a server multi-client architecture & U & U & U & Y & Y & Y \\
\hline 
\textbf{Open Source} & N & N & N & Y & Y & Y \\
\hline
\textbf{Well-maintained/Stable} & Y & Y & Y & Y & Y & Y \\
\hline
\textbf{Portability} & Y & Y & Y & Y, Windows, Linux & Y, Windows, Linux & Y, Windows, Linux\\
\hline
\textbf{Flexible API} & Y & Y & U & Y (2) & Y & Y\\
\hline
\end{tabular}
\begin{tablenotes}
    \item[1] Y=supported, N = not supported, U = unknown
    \item[2] (1) See section 4.4 for details about Carla.
    \item[3] (2) See section 4.5 for details about Gazebo
    \item[4] (3) See section 4.6 for details about LGSVL
\end{tablenotes}
\end{table*}


==> content/06_Challenges.tex <==
\section{Challenges}
The automotive simulators have come a long way. Although simulation has now become a cornerstone in the development of self-driving cars, common standards to evaluate simulation results is lacking. For example, the Annual Mileage Report submitted to the California Department of Motor Vehicle by the key players such as Waymo, Cruise, and Tesla does not include the sophistication and diversity of the miles collected through simulation \cite{amr}. It would be more beneficial to have simulation standards that could help make a more informative comparison between various research efforts. 

Further, we are not aware of any simulators that are currently capable of testing the concept of connected vehicles, where vehicles communicate with each other and with the infrastructure. However, there are test beds available such as the ones mentioned in the report \cite{dotintelligent} from the US Department of Transportation.

In addition, current simulators, for instance CARLA and LGSVL, are on-going projects and add the most recent technologies. Therefore, the user may encounter with undocumented errors or bugs. Therefore, the community support is quite important which can improve the quality of open source simulators and ADAS tests.

==> content/07_RelatedWork.tex <==
\section{Related Work}
\label{sec:related}
There are many other simulators available that are not explicitly reviewed in this paper. For example, RoadView is a traffic scene modelling simulator built using image sequences and the road Global Information System (GIS) data \cite{zhang2014roadview}. \cite{banerjee2019development} provides an in-depth review of CARLA simulator and how it can be used to test autonomous driving algorithms. Similarly, \cite{fadaie2019state}, \cite{chao2020survey}, and \cite{figueiredo2009approach} provide review of various other automotive and robotic simulators. \cite{tang2017distributed} discusses a distributed simulation platform for testing.


==> content/Applications.tex <==
\section{Applications}
Cooperation between Autonomous Vehicles (AVs) and Autonomous Delivery Robots (ADRs) is an interesting topic that AVs could first deliver goods to a community or campus, then ADRs could be responsible for the last mile delivery to the customers\cite{co}. Our simulator could test this process in terms of communication and planning between an ADR and an AV.  Fig. 5 shows our AV Hydro and ADR ZebraT, which can share the map and sensing data between each other to implement cooperation tasks. Although this is a new topic and not too much work has been done, the potential impact that it could bring to society still deserves more effort from developers and researchers. 



==> content/content/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}
With the push from cloud services and pull from IoT~\cite{shi2016edge},
we envision that the edge of the network is changing from
data consumer to data producer as well as data consumer$\footnote{\href{https://www.thecarlab.org/outcomes/software}{https://www.thecarlab.org/outcomes/software}}$.
In this paper, we attempt to contribute the concept of edge
computing. We start from the analysis of why we need
edge computing, then we xxxxxx

The remaining parts of this paper are organized as follows.
Section II discusses the need for edge computing as well as
gives the definition of edge computing. In Section III, we
show some edge computing case studies. Section IV presents
the possible challenges and opportunities. Finally, this paper
concludes in Section V.

==> content/content/02_Motivations.tex <==
\section{Motivation}
\label{sec:motivation}

\noindent \textbf{Pull From IoT: }
Raw data produced by them will be enormous,
making conventional cloud computing not efficient enough to
handle all these data. This means most of the data produced
by IoT will never be transmitted to the cloud, instead it will
be consumed at the edge of the network.
In general, EdgeWare is different from Rocket in terms of six aspects, which is shown in Table~\ref{tab:hardwarecost}. 


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht]
\centering
\caption{Hardware Equipment of Autonomous Vehicles.}
\label{tab:hardwarecost}
\scalebox{0.77}{
\begin{threeparttable}[b]
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Hardware Equipment} & \multicolumn{2}{c|}{Unit Price} \\ \hline
\multicolumn{2}{|c|}{\multirow{2}{*}{Communication Device}} & DSRC & \$17,600 \\ \cline{3-4} 
\multicolumn{2}{|c|}{} & LTE/5G/C-V2X & \$177 \\ \hline
\multicolumn{2}{|c|}{Computation Device} & \begin{tabular}[c]{@{}c@{}}Consists of a PC, a hard drive,\\ a graphics card, and other devices\end{tabular} & \$5000 \\ \hline
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}Vehicle Electronic\\ Control Unit (ECU)\end{tabular}} & Each vehicle has 50 to 100 ECUs & \$320 each \\ \hline
\multicolumn{2}{|c|}{Power Supply} & \multicolumn{2}{c|}{\$24,300} \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\\\\\\Sensor\end{tabular}} & Camera & \multicolumn{2}{c|}{\$6000} \\ \cline{2-4} 
 & LiDAR & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\$8,5000 (installed on the top, \\ 360-degree field of view)\\ + \$8,000 * 4 (4 small ones installed \\ in 4 corners)\end{tabular}} \\ \cline{2-4} 
 & Radar & \multicolumn{2}{c|}{\$500 each * 6} \\ \cline{2-4} 
 & Other & \multicolumn{2}{c|}{Eg. inertial measurement unit, \$4,000} \\ \hline
\end{tabular}
\begin{tablenotes}
     \item[1] Data listed as of August 2020. 
     \item[2] Use the following web tools to customize a table: 
     \item[] \href{https://www.tablesgenerator.com/latex_tables}{https://www.tablesgenerator.com/latex\_tables} 
\end{tablenotes}
\end{threeparttable}
}
\vspace{-0.6 cm}
\end{table}

Reliability is also a key challenge at the edge of the network. We identify the challenges
in reliability from the different views of service, system, and
data here.

\begin{itemize}
\item[\ding{118}] From the service point of view, it is sometimes very hard to identify the reason for a service failure accurately at
field. For example, if an air conditioner is not working, a
potential reason could be that a power cord is cut, compressor failure, or even a temperature controller has run
out of battery. A sensor node could have lost connection very easily to the system due to battery outage, bad
connection condition, component wear out, etc. At the
edge of the network, it is not enough to just maintain a
current service when some nodes lose connection, xxxxxx
\item[\ding{118}] From the system point of view, it is very important for
the edgeOS to maintain the network topology of the
whole system, and each component in the system is
able to send status/diagnosis information to the edgeOS.
With this feature, services such as failure detection, thing
replacement, and data quality detection could be easily
deployed at the system level.
\item[\ding{118}] From the data point of view, reliability challenge rise
mostly from the data sensing and communication part.
As previously researched and discussed, things at the
edge of the network could fail due to various reasons and
they could also report low fidelity data under unreliable
condition such as low battery level.
\end{itemize}


==> content/content/03_Architecture.tex <==
\section{Architecture}
\label{sec:Architecture}
If all the data needs to be sent to the cloud
for processing, the response time would be too long. Not to
mention that current network bandwidth and reliability would
be challenged for its capability of supporting a large number
of vehicles in one area. In this case, the data needs to be processed at the edge for shorter response time, more efficient
processing and smaller network pressure.
\weisong{give more details about xxxxx}

\begin{equation}
\begin{array}{c}
  S = \binom{N}{n},A_{k} = \binom{M}{k}\cdot \binom{N-M}{n-k} \\ \\
  P\left ( A_{k}\right ) = \frac{\binom{M}{k}\cdot \binom{N-M}{n-k}}{\binom{N}{n}} 
\end{array}
\end{equation}

Use the following web tool to get the formula in latex format:
\href{https://www.latexlive.com/}{https://www.latexlive.com/} 

==> content/content/04_CaseStudy.tex <==
\section{Case Study}
\label{sec:case}
In this section, we give several case studies where edge
computing could shine to further illustrate our vision of edge
computing.

\subsection{Cloud Offloading}
\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figures/Equinox.pdf}
\caption{Insert a figure.}
\label{system-design}
\end{figure}

In the traditional content delivery network, only the data is
cached at the edge servers. This is based on the fact that the
content provider provides the data on the Internet, which is
true for the past decades. In the IoT, the data is produced and
consumed at the edge. Thus, in the edge computing paradigm,
not only data but also operations applied on the data should
be cached at the edge.

\subsection{Video Analytics}
The widespread of mobilephones and network cameras
make video analytics an emerging technology. Cloud computing is no longer suitable for applications that requires video
analytics due to the long data transmission latency and privacy
concerns. Here we give an example of finding a lost child
in the city.

==> content/content/05_Evaluation.tex <==
\section{Evaluation and Observation}
\label{sec:evaluation}
From the system point of view, it is very important for
the edgeOS to maintain the network topology of the
whole system, and each component in the system is
able to send status/diagnosis information to the edgeOS.
With this feature, services such as failure detection, thing
replacement, and data quality detection could be easily
deployed at the system level.


==> content/content/06_RelatedWork.tex <==
\section{Related Work}
\label{sec:related}
In edge computing, we have multiple layers with different
computation capability~\cite{Li:2013:Bugu,Bing:eCope}. Workload allocation becomes a big
issue. We need to decide which layer to handle the workload
or how many tasks to assign at each part. There are multiple allocation strategies to complete a workload, for instances, xxxxxx

==> content/content/07_Conclusion.tex <==
\section{Conclusion Remarks}
\label{sec:conclusion}
Nowadays, more and more services are pushed from the
cloud to the edge of the network because processing data at
the edge can ensure shorter response time and better reliability.
Moreover, bandwidth could also be saved if xxxxxx
